The obstacle problem for linear scalar conservation laws with constant velocity

In this contribution, we present a novel approach for solving the obstacle problem for (linear) conservation laws. Usually, given a conservation law with an initial datum, the solution is uniquely determined. How to incorporate obstacles, i.e., inequality constraints on the solution so that the resulting solution is still "physically reasonable" and obeys the obstacle, is unclear. The proposed approach involves scaling down the velocity of the conservation law when the solution approaches the obstacle. We demonstrate that this leads to a reasonable solution and show that, when scaling down is performed in a discontinuous fashion, we still obtain a suitable velocity - and the solution satisfying a discontinuous conservation law. We illustrate the developed solution concept using numerical approximations.

==> definitions_sn.tex <==
\newcommand{\x}{\boldsymbol x}
\newcommand{\z}{\boldsymbol z}
\newcommand{\y}{\boldsymbol y}
\newcommand{\h}{\boldsymbol h}
\newcommand{\q}{\boldsymbol q}
\newcommand{\e}{\mathrm{e}}
\newcommand{\blambda}{\boldsymbol \lambda}
\newcommand{\bgamma}{\boldsymbol \gamma}
\newcommand{\R}{\mathbb R}
\newcommand{\N}{\mathbb N}
\newcommand{\Z}{\mathbb Z}
\newcommand{\M}{\mathbf{M}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bI}{\boldsymbol I}
\newcommand{\bJ}{\boldsymbol J}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\gammae}{\gamma^{\text{e}}}
\newcommand{\gammac}{\gamma^{\text{c}}}
\newcommand{\gammaz}{\gamma^{\text{z}}}
\newcommand{\gammaep}{\gamma^{\text{ep}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\mA}{\mathcal A}
\newcommand{\mB}{\mathcal B}
\newcommand{\mC}{\mathcal C}
\newcommand{\mD}{\mathcal D}
\newcommand{\mDMM}{\mathcal D_{M,M'_{\nu}}}
\newcommand{\mE}{\mathcal E}
\newcommand{\mF}{\mathcal F}
\newcommand{\mFnueps}{\mF_{_{\!\!\nu,\eps}}}
\newcommand{\mEF}{\mathcal{EF}}
\newcommand{\mEFx}{\mathcal{EF}x}
\newcommand{\mS}{\mathcal S}
\newcommand{\mEMM}{\mathcal E_{M}(M'_{\nu})}
\newcommand{\GMM}{\Gamma_{\scriptscriptstyle \!\!M'}^{\scriptscriptstyle M}}

\newcommand{\mG}{\mathcal G}
\newcommand{\mH}{\mathcal H}
\newcommand{\nceil}{\ensuremath{\left\lceil\frac{N}{\eta}\right\rceil}}
\newcommand{\Wq}{W_{\!\eta}[q_{\eta}]}

\newcommand{\cX}{{\boldsymbol{\mathcal X}}}
\newcommand{\cY}{{\boldsymbol{\mathcal Y}}}
\newcommand{\cQ}{{\boldsymbol{\mathcal Q}}}
\newcommand{\bt}{{\boldsymbol{t}}}
\newcommand{\cE}{{\boldsymbol{\mathcal E}}}
\newcommand{\boldeta}{\boldsymbol{\eta}}
\newcommand{\cA}{\mathcal A}
\newcommand{\cB}{\mathcal B}
\newcommand{\cC}{\mathcal C}
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cP}{\mathcal P}
\newcommand{\cK}{\mathcal K}
\newcommand{\cI}{\mathcal I}
\newcommand{\cO}{\mathcal O}
\newcommand{\xie}{\xi_\eta}
\newcommand{\We}{W_\eta}
\newcommand{\Weo}{W_{\eta,0}}
\newcommand{\qe}{q_\eta}


\newcommand{\cRM}{\mathcal{RM}}
\newcommand{\invp}{{{\!\!\scriptscriptstyle\frac{1}{p}}}}
\newcommand{\weakstar}{\overset{*}{\rightharpoonup}}
\newcommand{\qpc}{q_{\scriptscriptstyle\mathrm{pc}}}
\newcommand{\id}{\ensuremath{\mathrm{Id}}}
\newcommand{\CM}{C_{\!\M}}

\newcommand{\mbM}{\mathbb M}

\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\renewcommand{\:}{\mathrel{\coloneqq}}
\renewcommand{\=}{\ensuremath{\eqqcolon}}
\newcommand{\equivd}{\ensuremath{\vcentcolon\equiv}}
\newcommand{\OT}{{\Omega_{T}}}
\newcommand{\OTeta}{{\Omega_{T}^{\eta}}}

\newcommand{\Ot}{{\Omega_{t}}}
\newcommand{\OTs}{\Omega_{T^*}}
\newcommand{\Vmax}{V_{\text{max}}}
\newcommand{\I}{\ensuremath{\int\limits}}
%\newcommand{\I}{\ensuremath{\int}}
\newcommand{\loc}{\textnormal{loc}}
\newcommand{\cc}{\text{c}}

\newcommand{\mTl}{\mathcal T_{\!_{<}}\!}
\newcommand{\mTg}{\mathcal T_{\!_{>}}\!}
\newcommand{\mTe}{\mathcal T_{\!_{=}}\!}


\newcommand{\dd}{\ensuremath{\,\mathrm{d}}}
\newcommand{\ddx}{\ensuremath{\tfrac{d}{dx}}}
\newcommand{\ddy}{\ensuremath{\tfrac{d}{dy}}}
\newcommand{\ddt}{\ensuremath{\tfrac{d}{dt}}}
\newcommand{\ddZ}{\ensuremath{\tfrac{d}{dz}}}
\newcommand{\dde}{\ensuremath{\partial_1}}
\newcommand{\ddz}{\ensuremath{\partial_2}}
\newcommand{\ddd}{\ensuremath{\partial_3}}
\newcommand{\F}{\ensuremath{\boldsymbol{F}}}
\newcommand{\G}{\ensuremath{\boldsymbol{G}}}
\newcommand{\D}{\ensuremath{\mathrm{D}}}
\newcommand{\Vad}{\ensuremath{V_{\text{ad}}}}
\newcommand{\Had}{\ensuremath{H_{\text{ad}}}}
\newcommand{\Lad}{\ensuremath{\Lambda_{\text{ad}}}}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator*{\esslim}{ess\,lim}
\DeclareMathOperator*{\argmin}{arg-\min}
\DeclareMathOperator*{\argmax}{arg-\max}
\newcommand{\todoA}[1]{\todo[inline,color=green!30!white]{#1}}
\newcommand{\todoL}[1]{\todo[inline,color=red!20!white]{#1}}
\newcommand{\todoM}[1]{\todo[inline,color=blue!20!white]{#1}}
\newcommand{\Cb}{\ensuremath{C_{\text{b}}}}
\newcommand{\nd}{\hspace{-0.5em}}
\newcommand{\md}{\hspace{-2em}}
\newcommand{\bA}{{\color{orange}\textbf{A}}}
\newcommand{\bL}{{\color{green}\textbf{L}}}
\newcommand{\bM}{{\color{blue}\textbf{M}}}

\newcommand{\bQ}{\ensuremath{\boldsymbol{\mathcal Q}}}
\newcommand{\bq}{\ensuremath{\boldsymbol{q}}}
\newcommand{\bX}{\ensuremath{\boldsymbol{\mathcal X}}}
\newcommand{\bY}{\ensuremath{\boldsymbol{\mathcal Y}}}
\newcommand{\bZ}{\ensuremath{\boldsymbol{\mathcal Z}}}
\newcommand{\bpsi}{\ensuremath{\boldsymbol{\psi}}}
\newcommand{\bPsi}{\ensuremath{\boldsymbol{\Psi}}}
\newcommand{\bphi}{\ensuremath{\boldsymbol{\phi}}}
\newcommand{\bdel}{\ensuremath{\boldsymbol{\delta}}} 
\newcommand{\btau}{\ensuremath{\boldsymbol{\tau}}} 
\newcommand{\odel}{\ensuremath{\overline{\delta}}} 

\newcommand{\bcI}{\ensuremath{\boldsymbol{\mathcal I}}}
\renewcommand{\epsilon}{\varepsilon}

\newcommand{\redC}[1]{\textcolor{red}{#1}} % Erase me later; shortcut for red comments


\crefname{ineq}{Inequality}{Inequalities}
\creflabelformat{ineq}{#2{(#1)}#3}
\crefname{assumption}{Assumption}{Assumptions}

